Efficient Diffusion Models: A Comprehensive Survey from Principles to Practices

As one of the most popular and sought-after generative models in the recent years, diffusion models have sparked the interests of many researchers and steadily shown excellent advantage in various generative tasks such as image synthesis, video generation, molecule design, 3D scene rendering and multimodal generation, relying on their dense theoretical principles and reliable application practices. The remarkable success of these recent efforts on diffusion models comes largely from progressive design principles and efficient architecture, training, inference, and deployment methodologies. However, there has not been a comprehensive and in-depth review to summarize these principles and practices to help the rapid understanding and application of diffusion models. In this survey, we provide a new efficiency-oriented perspective on these existing efforts, which mainly focuses on the profound principles and efficient practices in architecture designs, model training, fast inference and reliable deployment, to guide further theoretical research, algorithm migration and model application for new scenarios in a reader-friendly way. \url{https://github.com/ponyzym/Efficient-DMs-Survey}

==> tables/table1.tex <==
\begin{table}[ht]
\centering
\setlength{\tabcolsep}{2pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lc|cccccccccccccc}
\toprule
\textbf{Model}                                     & \textbf{LLM Backbone}       & \textbf{VQA$^\text{v2}$} & \textbf{GQA}  & \textbf{SQA$^\text{I}$} & \textbf{VQA$^\text{T}$} & \textbf{VizWiz} & \textbf{MMMU}      & \textbf{MathV} & \textbf{MME$^\text{P}$}   & \textbf{MME$^\text{C}$}   & \textbf{MMB}  & \textbf{SEED}      & \textbf{POPE} & \textbf{LLAVA$^\text{W}$} & \textbf{MM-Vet} \\ \midrule
Flamingo~\cite{alayrac2022flamingo}                & Chinchilla-7B      & -     & -    & -    & -    & 28.8   & -         & -     & -      & -      & -    & -         & -    & -      & -      \\
BLIP-2~\cite{li2023blip2}                  & Flan-T5XXL(13B)    & 65.0  & 44.7 & 61.0 & 42.5 & 19.6   & -         & -     & 1293.8 & 290.0  & -    & -/46.4    & 85.3 & 38.1   & 22.4   \\
LLaVA~\cite{liu2023llava}                 & Vicuna-13B         & -     & 41.3 & -    & 38.9 & -      & -         & -     & -      & -      & -    & -         & -    & -      & -      \\
MiniGPT-4~\cite{zhu2023minigpt4}          & Vicuna-13B         & -     & 30.8 & -    & 19.4 & -      & -         & -     & -      & -      & -    & -         & -    & -      & -      \\
InstructBLIP~\cite{dai2024instructblip}   & Vicuna-13B         & -     & 49.5 & 63.1 & 50.7 & 33.4   & -         & -     & 1212.8 & 291.8  & -    & -         & 78.9 & 58.2   & 25.6   \\
Qwen-VL-Chat~\cite{bai2023qwen-vl}        & Qwen-7B            & 78.2$^*$  & 57.5$^*$ & 68.2 & 61.5 & 38.9   & 35.9/32.9 & -     & 1487.5 & 360.7  & 60.6 & -/58.2    & -    & -      & -      \\
LLaVA-1.5~\cite{liu2023llava1.5}          & Vicuna-1.5-13B     & 80.0$^*$  & 63.3$^*$ & \color{blue}\textbf{71.6} & 61.3 & 53.6   & -         & -     & 1531.3 & 295.4  & 67.7 & -/68.2    & 85.9 & \color{blue}\textbf{70.7}   & 35.4   \\
MiniGPT-v2-Chat~\cite{chen2023minigpt-v2} & LLaMA-2-Chat-7B    & -     & 58.8 & -    & 52.3 & 42.4   & -         & -     & -      & -      & -    & -         & -    & -      & -      \\
InternVL-Chat~\cite{chen2023internvl}                             & Vicuna-13B         & 81.2$^*$  & \textcolor{blue}{\textbf{66.6}}$^*$ & -    & 61.5 & \color{blue}58.5   & -         & -     & \color{blue}\textbf{1586.4} & -      & -    & -         & \color{blue}\textbf{87.6} & -      & -      \\
Emu2-Chat~\cite{sun2023generative}                                 & LLaMA-33B          & \textcolor{blue}{\textbf{84.9}}$^*$  & 65.1$^*$ & -    & 66.6$^*$    & 54.9   & -/34.1      & -     & -      & -      & -    & 62.8      & -    & -      & 48.5   \\
Gemini Pro~\cite{team2023gemini}                                & -                  & 71.2  & -    & -    & 74.6 & -      & 47.9/–    & 45.2  & -      & 436.79 & 73.6 & –/70.7    & -    & -      & 64.3   \\
Gemini Ultra~\cite{team2023gemini}                              & -                  & 77.8  & -    & -    & \color{blue}\textbf{82.3} & -      & \color{blue}\textbf{59.4/–}    & \color{blue}\textbf{53.0}    & -      & -      & -    & -         & -    & -      & -      \\
GPT4V~\cite{achiam2023gpt}                                     & -                  & 77.2  & -    & -    & 78.0 & -      & 56.8/55.7 & 49.9  & -      & \color{blue}\textbf{517.14} & \color{blue}\textbf{75.8} & \color{blue}\textbf{67.3/69.1} & -    & -      & \color{blue}\textbf{67.6}  \\ \midrule
MobileVLM~\cite{chu2023mobilevlmv1}       & MobileLLaMA (2.7B) & -     & 59.0$^*$ & 61.0 & 47.5 & -      & -         & -     & 1288.9 & -      & 59.6 & -         & 84.9 & -      & -      \\
LLaVA-Phi~\cite{zhu2024llava-phi}         & Phi-2 (2.7B)       & 71.4$^*$  & -    & 68.4 & 48.6 & 35.9   & -         & -     & 1335.1 & -      & 59.8 & -         & 85.0 & -      & 28.9   \\
Imp-v1~\cite{imp2024}                     & Phi-2 (2.7B)       & 79.5  & -    & 70.0 & 59.4 & -      & -         & -     & 1434.0 & -      & 66.5 & -         & \color{red}\textbf{88.0} & -      & 33.1   \\
TinyLLaVA~\cite{zhou2024tinyllava}        & Phi-2 (2.7B)       & 79.9$^*$  & 62.0$^*$ & 69.1 & 59.1 & -      & -         & -     & 1464.9 & -      & 66.9 & -         & 86.4 & 75.8   & 32.0   \\
Bunny~\cite{he2024bunny}                  & Phi-2 (2.7B)       & 79.8  & 62.5 & 70.9 & -    & -      & 38.2/33.0 & -     & 1488.8 & 289.3  & 68.6 & 62.5/-    & 86.8 & -      & -      \\
Gemini   Nano-2~\cite{team2023gemini}     & -                  & 67.5  & -    & -    & 65.9 & -      & 32.6/-    & 30.6  & -      & -      & -    & -         & -    & -      & -      \\
MobileVLM-v2~\cite{chu2024mobilevlmv2} & MobileLLaMA(2.7B)  & -     & 61.1 & 70.0 & 57.5 & -      & -         & -     & 1440.5 & -      & -    & -         & 84.7 & -      & -      \\
MoE-LLaVA~\cite{lin2024moe-llava}    & Phi-2 (2.7B)       & 79.9$^*$  & 62.6$^*$ & 70.3 & 57.0 & 43.7   & -         & -     & 1431.3 & -      & 68.0 & -         & 85.7 & -      & 35.9   \\
Cobra~\cite{zhao2024cobra}                & Mamba-2.8B  & 75.9  & 58.5 & -    & 46.0 & \color{red}\textbf{52.0}   & -         & -     & -      & -      & -    & -         & \color{red}\textbf{88.0} & -      & -      \\
Mini-Gemini~\cite{li2024mini-gemini}      & Gemma-2B           & -     & -    & -    & 56.2 & -      & 31.7/29.1 & 29.4  & 1341.0 & 312.0  & 59.8 & -         & -    & -      & 31.1   \\
Vary-toy~\cite{wei2024vary-toy}           & Qwen-1.8B          & -     & -    & -    & -    & -      & -         & -     & -      & -      & -    & -         & -    & -      & 29.0   \\
TinyGPT-V~\cite{yuan2023tinygpt-v}        & Phi-2 (2.7B)       & -     & 33.6 & -    & -    & 24.8   & -         & -     & -      & -      & -    & -         & -    & -      & -      \\
SPHINX-Tiny~\cite{gao2024sphinx}          & TinyLlama-1.1B     & -     & -    & -    & 57.8 & -      & -         & 26.4  & 1261.2 & 242.1  & 56.6 & 17.1/-    & 82.2 & 52.3   & 23.8   \\
ALLaVA-Longer~\cite{chen2024allava}       & Phi-2 (2.7B)                     & -        & 50.0 & -     & 50.3  & -      & 33.2/-    & -     & \multicolumn{2}{c}{1564.6$^\dagger$} & 64.6 & -         & -    & 71.7    & 35.5   \\
MM1-3B~\cite{mckinzie2024mm1}    & MM1-3B                  & \color{red}\textbf{82.5}  & -    & 76.1 & \color{red}\textbf{72.9} & -      & 38.6/35.7 & 32.6  & 1469.4 & 303.1  & 70.8 & 63.9/69.4 & 87.6 & \color{red}\textbf{76.8}   & \color{red}\textbf{42.2}   \\
LLaVA-Gemma~\cite{hinck2024llava-gemma}   & Gemma-2b-it        & 71.4  & 58.7 & -    & -    & -      & -         & -     & 1133.0 & 307.0  & -    & -         & 85.3 & -      & 19.1   \\
Mipha-3B~\cite{zhu2024mipha}              & Phi-2 (2.7B)       & 81.3$^*$  & \textcolor{red}{\textbf{63.9}}$^*$ & 70.9 & 56.6 & 47.5   & -         & -     & 1488.9 & 295.0  & 69.7 & -         & 86.7 & -      & 32.1   \\
VL-Mamba~\cite{qiao2024vlmamba}           & Mamba-2.8B     & 76.6  & 56.2 & 65.4 & 48.9 & -      & -         & -     & 1369.6 & -      & 57.0 & -         & 84.4 & -      & 32.6   \\ 
MiniCPM-V 2.0\cite{minicpm-v}                          & MiniCPM-2.4B       & -        & -    & -     & 74.1  & -      & 38.2/-    & \color{red}\textbf{38.7}  & \multicolumn{2}{c}{1808.6$^\dagger$} & 69.6 & -         & -    & -       & -   \\ 
DeepSeek-VL~\cite{lu2024deepseekvl}           & DeepSeek-LLM-1B     & -  & - & - & - & -      & 32.2/-         & 31.1     & - & -      & 64.6 & -/66.7         & 87.6 & -      & 36.8   \\ 
KarmaVLM\cite{karmavlm}           & Qwen1.5-0.5B     & -  & - & 53.86 & 45.25 & -      & -         & -     & - & -      & 55.8 & -        & - & 47.5      & -   \\ 
moondream2\cite{moondream}           & Phi-1.5(1.3B)     & 77.7  & 61.7 & - & 49.7 & -      & -         & -     & - & -      & - & -        & - & -      & -   \\ 
Bunny-v1.1-4B\cite{he2024bunny}           & Phi-3-Mini-4K     & 81.7  & 63.4 & \color{red}\textbf{76.3} & - & -      & \color{red}\textbf{40.2/38.8}         & -     & \color{red}\textbf{1503.9} & \color{red}\textbf{362.9}      & \color{red}\textbf{74.1} & \color{red}\textbf{64.6/71.7}        & 87.0 & -      & -   \\ \bottomrule
\end{tabular}% 
}
\caption{Comparison of mainstream MLLMs and efficient MLLMs on 14 VL benchmarks. VQA$^\text{v2}$~\cite{goyal2017vqav2}; 
VQA$^\text{T}$: TextVQA~\cite{singh2019vqat}; GQA~\cite{hudson2019gqa}; SQA$^\text{I}$: ScienceQA-IMG~\cite{lu2022scienceQA}; VizWiz~\cite{gurari2018vizwiz}; MMMU~\cite{yue2023mmmu}; MathV: MathVista~\cite{lu2023mathvista}; MME$^\text{P/C}$: the Perception/Cognition split of MME~\cite{fu2024mme}; MMB: MMBench~\cite{liu2023mmbench}; SEED: SEED-Bench~\cite{li2023seedbench}; POPE~\cite{li2023pope}; LLaVA$^\text{W}$: LLaVA-Bench (In-the-Wild)~\cite{liu2023llava}; MM-Vet~\cite{yu2023mmvet}. The two numbers reported in MMMU denote the performance on the val and test split, respectively. The two numbers reported in SEED denote the performance on the whole SEED-Bench and the image part, respectively. $^\dagger$ denotes the combined points of two splits. $^*$ indicates that training images of the datasets are observed during training.The \textcolor{red}{\textbf{red}} denotes the highest result of efficient MLLMs, and the \textcolor{blue}{\textbf{blue}} denotes that of large-scale MLLMs.}
\label{benchmarktable}
\end{table}



==> tables/table2.tex <==
\begin{table}[ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Vision Encoder}}                   & \multicolumn{2}{c}{LLM}            & \multirow{2}{*}{\textbf{Vision-LLM Projector}} \\
                       & Variants               & Resolution & Parameter Size & Variants          & Parameter Size &                                              \\ \midrule
MobileVLM~\cite{chu2023mobilevlmv1}              & CLIP ViT-L/14~\cite{radford2021clip}          & 336        & 0.3B           & MobileLLaMA\cite{chu2023mobilevlmv1}       & 2.7B           & LDP\cite{chu2023mobilevlmv1}                                          \\
LLaVA-Phi~\cite{zhu2024llava-phi}              & CLIP ViT-L/14~\cite{radford2021clip}          & 336        & 0.3B           & Phi-2\cite{javaheripi2023phi}             & 2.7B           & MLP                                          \\
Imp-v1~\cite{imp2024}                 & SigLIP~\cite{zhai2023siglip}                 & 384        & 0.4B           & Phi-2\cite{javaheripi2023phi}             & 2.7B           & -                                            \\
TinyLLaVA~\cite{zhou2024tinyllava}              & SigLIP-SO~\cite{zhai2023siglip}              & 384        & 0.4B           & Phi-2\cite{javaheripi2023phi}             & 2.7B           & MLP                                          \\
Bunny~\cite{he2024bunny}                  & SigLIP-SO~\cite{zhai2023siglip}              & 384        & 0.4B           & Phi-2\cite{javaheripi2023phi}             & 2.7B           & MLP                                          \\
MobileVLM-v2-3B~\cite{chu2024mobilevlmv2}        & CLIP ViT-L/14~\cite{radford2021clip}          & 336        & 0.3B           & MobileLLaMA\cite{chu2024mobilevlmv2}       & 2.7B           & LDPv2\cite{chu2024mobilevlmv2}                                        \\
MoE-LLaVA-3.6B~\cite{lin2024moe-llava}         & CLIP-Large~\cite{radford2021clip}             & 384        & -              & Phi-2\cite{javaheripi2023phi}             & 2.7B           & MLP                                          \\
Cobra~\cite{zhao2024cobra}                  & \makecell[c]{DINOv2~\cite{oquab2023dinov2} \\SigLIP-SO~\cite{zhai2023siglip}}     & 384        & 0.3B+0.4B      & Mamba-2.8b-Zephyr\cite{gu2023mamba} & 2.8B           & MLP                                          \\
Mini-Gemini~\cite{li2024mini-gemini}            & CLIP-Large~\cite{radford2021clip}             & 336        & -              & Gemma\cite{gemmateam2024gemma}             & 2B             & MLP                                          \\
Vary-toy~\cite{wei2024vary-toy}               & CLIP~\cite{radford2021clip}                   & 224        & -              & Qwen\cite{bai2023qwen}              & 1.8B           & -                                            \\
TinyGPT-V~\cite{yuan2023tinygpt-v}               & EVA~\cite{fang2023eva}                    & 224/448    & -              & Phi-2\cite{javaheripi2023phi}             & 2.7B           & Q-Former~\cite{li2023blip2}                                     \\
SPHINX-Tiny~\cite{gao2024sphinx}            & \makecell[c]{DINOv2~\cite{oquab2023dinov2} \\CLIP-ConvNeXt~\cite{liu2022convnet}} & 448        & -              & TinyLlama\cite{zhang2024tinyllama}         & 1.1B           & -                                            \\
ALLaVA-Longer~\cite{chen2024allava}          & CLIP-ViT-L/14~\cite{radford2021clip}          & 336        & 0.3B           & Phi-2\cite{javaheripi2023phi}             & 2.7B           & -                                            \\
MM1-3B-MoE-Chat~\cite{mckinzie2024mm1}        & CLIP$_\text{DFN}$-ViT-H~\cite{fang2023data}          & 378        & -              & -                  & 3B$^*$             & C-Abstractor~\cite{cha2023honeybee}                                 \\
LLaVA-Gemma~\cite{hinck2024llava-gemma}            & DinoV2~\cite{oquab2023dinov2}                 & -          & -              & Gemma-2b-it\cite{gemmateam2024gemma}       & 2B             & -                                            \\
Mipha-3B~\cite{zhu2024mipha}               & SigLIP~\cite{zhai2023siglip}                 & 384        & -              & Phi-2\cite{javaheripi2023phi}             & 2.7B           & -                                            \\
VL-Mamba~\cite{qiao2024vlmamba}               & SigLIP-SO~\cite{zhai2023siglip}                 & 384        & -              & Mamba-2.8B-Slimpj\cite{gu2023mamba}             & 2.8B           & VSS-L2\cite{qiao2024vlmamba}                                            \\
MiniCPM-V 2.0\cite{minicpm-v}              & SigLIP~\cite{zhai2023siglip}                 & -        & 0.4B              &  MiniCPM\cite{hu2024minicpm}             & 2.4B           & Perceiver Resampler~\cite{alayrac2022flamingo}                                            \\ 
DeepSeek-VL~\cite{lu2024deepseekvl}              & SigLIP-L~\cite{zhai2023siglip}                 & 384        & 0.4B              &  DeepSeek-LLM\cite{deepseek-llm}             &  1.3B           & MLP                                            \\ 
KarmaVLM\cite{karmavlm}              & SigLIP-SO~\cite{zhai2023siglip}                 & 384        & 0.4B              &  Qwen1.5\cite{bai2023qwen}             &  0.5B           & -                                           \\
moondream2\cite{moondream}              & SigLIP\cite{zhai2023siglip}                 & -        & -              &  Phi-1.5\cite{li2023phi}             &  1.3B           & -                                           \\ 
Bunny-v1.1-4B\cite{he2024bunny}              & SigLIP\cite{zhai2023siglip}                 & 1152$^\dagger$        & -              &  Phi-3-Mini-4K\cite{abdin2024phi3}             &   3.8B           & -                                           \\ \bottomrule
\end{tabular}%
}
\caption{The summary of 17 mainstream efficient MMLMs. $^*$ indicates activated parameters.$^\dagger$:High resolution support is achieved with S$^\text{2}$-Wrapper\cite{shi2024S2}.}
\label{summarytable}
\end{table}


==> tables/table4.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=left,font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]

\begin{figure*}[ht]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                text centered,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=13em,font=\normalsize,}{},
            where level=2{text width=15em,font=\normalsize,}{},
            where level=3{text width=16em,font=\normalsize,}{},
            where level=4{text width=18em,font=\normalsize,}{},
            where level=5{text width=18em,font=\normalsize,}{},
            [
                \textbf{Efficient Vision}, ver
                [
                        \textbf{Compact Architecture}(\S\ref{subsec:ca}), fill=blue!10    
                        [
                        \textbf{Architecture Design Methods}, fill=blue!10
                        [
                             Reformer\cite{kitaev2020reformer}{,}
                             EfficientFormer\cite{li2022efficientformer}{,}
                             \\ EfficientFormerV2\cite{li2023rethinking}, leaf, text width=18em
                        ]
                        ]
                        [
                            \textbf{Architecture Search Methods}, fill=blue!10
                            [
                              Autoformer~\cite{chen2021autoformer}{,}
                              NASViT~\cite{gong2022nasvit}{,}
                              \\TF-TAS~\cite{zhou2022training}{,}
                              UniNet~\cite{liu2022uninet}, leaf, text width=18em
                            ]
                        ]
                        [
                            \textbf{Optimization of Attention}
                            \\\textbf{Mechanisms Methods}, fill=blue!10
                            [
                                PatchMerger~\cite{renggli2022learning}{,}
                                DynamicViT~\cite{rao2021dynamicvit}{,}
                                \\Sepvit~\cite{li2022sepvit}, leaf, text width=18em
                            ]
                        ] 
                    ]                  
                [
                        \textbf{Pruning}(\S\ref{subsec:pru}), fill=green!10
                        [
                            \textbf{Unstructured Pruning}, fill=green!10
                            [
                            Cap~\cite{kuznedelev2024cap}{,}
                            Cait~\cite{wang2023cait}, leaf, text width=18em
                            ]
                        ]
                        [
                            \textbf{Structured Pruning}, fill=green!10
                              [
                             WDPruning~\cite{yu2022width}{,}
                             X-Pruner~\cite{yu2023x}{,}
                              \\VTP\cite{zhu2021vision}{,}
                              PS-ViT\cite{tang2022patch}, leaf, text width=18em
                              ]
                        ]
                        [
                            \textbf{Hybrid Pruning}, fill=green!10
                              [
                             SPViT~\cite{kong2022spvit}{,}
                             ViT-Slim~\cite{chavan2022vision}, leaf, text width=18em
                              ]
                        ]
                    ]
                     [
                        \textbf{Knowledge Distillation}(\S\ref{subsec:kd}), fill=yellow!10
                        [
                            \textbf{Homomorphic KD}, fill=yellow!10
                            [
                            DeiT~\cite{touvron2021training}{,}
                            TinyViT~\cite{wu2022tinyvit}{,}
                            m2mKD~\cite{lo2024m2mkd}{,}
                            \\DeiT-Tiny~\cite{hao2022learning}{,}
                             MiniViT~\cite{zhang2022minivit}, leaf, text width=18em
                            ]
                        ]
                        [
                            \textbf{Heteromorphic KD}, fill=yellow!10
                            [
                            DearKD~\cite{chen2022dearkd}{,}
                            CiT~\cite{ren2022co}, leaf, text width=18em
                            ]
                        ]
                    ]
                [
                    \textbf{Quantization}(\S\ref{subsec:quant}), fill=orange!10
                    [
                        \textbf{Post-Training Quantization},  fill=orange!10
                        [
                        PTQ4ViT~\cite{yuan2022ptq4vit}{,}
                        APQ-ViT~\cite{ding2022towards}{,}
                        \\NoisyQuant~\cite{liu2023noisyquant}, leaf, text width=18em
                        ]
                    ]
                    [
                        \textbf{Quantization-Aware Training},  fill=orange!10
                         [
                        Quantformer~\cite{wang2022quantformer}
                        Bit-shrinking~\cite{lin2023bit}{,}
                        \\Q-ViT~\cite{li2022q}{,}
                         TerViT~\cite{xu2022tervit}{,}
                         BiViT~\cite{he2023bivit}{,}
                         \\PackQViT~\cite{dong2024packqvit}{,}
                         BinaryViT~\cite{le2023binaryvit}, leaf, text width=18em
                        ]
                    ]
                    [
                        \textbf{Hardware-Aware Quantization},  fill=orange!10
                         [
                        GPUSQ-ViT\cite{yu2023boost}{,}
                        Auto-ViT-Acc~\cite{li2022auto}, leaf, text width=18em
                        ]
                    ]
                ]
            ]
        \end{forest}
        }
    \vspace{-0mm}
    \caption{Organization of efficient vision advancements.}
    \label{fig:efficient Vision}
    \vspace{0mm}
\end{figure*}

==> tables/table5.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=left,font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]

\begin{figure*}[ht]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                text centered,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=10em,font=\normalsize,}{},
            where level=2{text width=12em,font=\normalsize,}{},
            where level=3{text width=16em,font=\normalsize,}{},
            where level=4{text width=18em,font=\normalsize,}{},
            where level=5{text width=18em,font=\normalsize,}{},
            [
                \textbf{Efficient LLM}, ver
                [
                        \textbf{Attention}(\S\ref{subsec:att}), fill=blue!10    
                        [
                        \textbf{Sharing-based Attention}, fill=blue!10
                            [
                            GQA~\citep{ainslie2023gqa}{,}
                            Multi-Query Attention\cite{shazeer2019fast}, leaf, text width=18em
                            ]
                        ]
                        [
                            \textbf{Feature Information}
                            \\ \textbf{Reduction}, fill=blue!10
                            [
                                Funnel-Transformer~\citep{dai2020funnel}{,}
                                \\Set Transformer\cite{lee2019settransformer}, leaf, text width=18em
                            ]
                        ]
                        [
                            \textbf{Approximate Attention}, fill=blue!10
                            [
                               Linformer~\cite{wang2020linformer}{,}
                               Performer\cite{choromanski2020masked}, leaf, text width=18em
                            ]
                        ]
                    ]                  
                [
                        \textbf{Framework}(\S\ref{subsec:fra}), fill=green!10
                        [
                            \textbf{Mixture of Experts}, fill=green!10
                            [
                            GShard\cite{lepikhin2020gshard}{,}
                            Switch Transformer \cite{fedus2022switch}, leaf, text width=18em
                            ]
                        ]
                        [
                            \textbf{Transformer-Alternative}
                            \\ \textbf{Architecture}, fill=green!10
                              [
                              RWKV\cite{peng2023rwkv}{,}
                              S4\cite{gu2021efficiently}{,}
                               \\DSS\cite{gupta2022diagonal}{,}
                               Mamba\cite{gu2023mamba}, leaf, text width=18em
                              ]
                        ]
                    ]
                     [
                        \textbf{Fine-tuning}(\S\ref{subsec:ft}), fill=yellow!10
                        [
                            \textbf{Parameter-Efficient} 
                            \\ \textbf{Fine-Tuning}, fill=yellow!10
                            [
                             LLM-Adapters \cite{hu2023llm}{,}
                            (IA)$^\text{3}$~\cite{liu2020tfew}{,}
                            \\LoRA-FA~\cite{zhang2023lora}{,}
                            DyLoRa~\cite{valipour2022dylora}, leaf, text width=18em
                            ]
                        ]
                        [
                            \textbf{Full-Parameter fine-tuning}, fill=yellow!10
                            [
                            LOMO~\cite{lv2023full}{,}
                            MeZO\cite{malladi2023mezo}, leaf, text width=18em
                            ]
                        ]
                    ]
            ]
        \end{forest}
        }
    \vspace{-0mm}
    \caption{Organization of efficient large language models advancements.}
    \label{fig:efficient LLMs}
    \vspace{0mm}
\end{figure*}

==> tables/table6.tex <==
\begin{table}[ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
\textbf{Dataset Name}   & \textbf{X Modality} & \textbf{\#.X} & \textbf{\#.T} & \textbf{\#.X-T}    & \textbf{Representative Publications}                                                                              \\ \midrule
CC3M~\cite{sharma2018conceptual}                    & Image               & 3.3M          & 3.3M          & 3.3M               & TinyGPT-V\cite{yuan2023tinygpt-v},MM1\cite{mckinzie2024mm1}                                                                                     \\ \arrayrulecolor{gray!50} \midrule
CC12M~\cite{changpinyo2021conceptual}                   & Image               & 12.4M         & 12.4M         & 12.4M              & MM1\cite{mckinzie2024mm1}                                                                                               \\ \midrule 
SBU~\cite{ordonez2011im2text}                     & Image               & 1M            & 1M            & 1M                 & TinyGPT-V\cite{yuan2023tinygpt-v}                                                                                         \\ \midrule
LAION-5B~\cite{schuhmann2022laion}                & Image               & 5.9B          & 5.9B          & 5.9B               & TinyGPT-V\cite{yuan2023tinygpt-v}                                                                                         \\\midrule
LAION-COCO\cite{schuhmann2021laion}              & Image               & 600M          & 600M          & 600M               & Vary-toy~\cite{wei2024vary-toy}                                                                                          \\\midrule
COYO \cite{kakaobrain2022coyo-700m}                  & Image               & 747M          & 747M          & 747M               & MM1\cite{mckinzie2024mm1}                                                                                               \\\midrule
COCO Caption\cite{chen2015microsoft}            & Image               & 164K          & 1M            & 1M                 & Vary-toy~\cite{wei2024vary-toy}                                                                                          \\\midrule
CC595k \cite{liu2023llava}                 & Image               & 595K          & 595K          & 595K               & \begin{tabular}[c]{@{}c@{}}MobileVLM~\cite{chu2023mobilevlmv1},LLaVA-Phi~\cite{zhu2024llava-phi},\\ LLaVA-Gemma~\cite{hinck2024llava-gemma},Mini-Gemini~\cite{li2024mini-gemini}\end{tabular}            \\\midrule
RefCOCO\cite{kazemzadeh2014referitgame}                & Image               & 20K           & 142K          & 142K               & Vary-toy~\cite{wei2024vary-toy}                                                                                          \\\midrule
DocVQA\cite{mathew2021docvqa}                  & Image               & 12K           & 50K           & 50K                & Vary-toy~\cite{wei2024vary-toy}                                                                                          \\\midrule
LLava-1.5-PT\cite{liu2023llava1.5}            & Image               & 558K          & 558K          & 558K               & \begin{tabular}[c]{@{}c@{}}Imp-v1~\cite{imp2024},MoE-LLaVA~\cite{lin2024moe-llava},\\ Vary-toy~\cite{wei2024vary-toy},Mipha~\cite{zhu2024mipha},\\ VL-Mamba~\cite{qiao2024vlmamba},Tiny-LLaVA~\cite{zhou2024tinyllava}\end{tabular} \\\midrule
ShareGPT4V-PT \cite{chen2023sharegpt4v}          & Image               & 1246K         & 1246K         & 1246K              & Tiny-LLava~\cite{zhou2024tinyllava},MobileVLM V2~\cite{chu2024mobilevlmv2}                                                                           \\\midrule
ShareGPT4   \cite{chen2023sharegpt4v}        & Image               & 100K          & 100K          & 100K               & ALLaVA~\cite{chen2024allava}                                                                                            \\\midrule
Bunny-pretrain-LAION-2M\cite{he2024bunny} & Image               & 2M            & 2M            & 2M                 & Bunny~\cite{he2024bunny}                                                                                             \\\midrule
ALLaVA-Caption-4V \cite{chen2024allava}      & Image               & 715K          & 715K          & 715K               & Mini-Gemini~\cite{li2024mini-gemini}, ALLaVA\cite{chen2024allava}                                                                               \\\midrule
MMC4 (Interleaved) \cite{zhu2024multimodal}     & Image               & 571M          & 43B           & 101.2M (Instances) & DeepSeek-VL~\cite{lu2024deepseekvl}                                                                                       \\\midrule \arrayrulecolor{black}
Obelics (Interleaved)\cite{laurenccon2024obelics}   & Image               & 353M          & 115M          & 141M (Instances)   & MM1\cite{mckinzie2024mm1}                                                \\ \bottomrule                                                  
\end{tabular}%
}
\caption{The statistics for common MLLM PT datasets.\#.X represents the quantity of X, \#.T represents the quantity of Text, and \#.X-T represents the quantity of X-Text pairs, where X can be Image, Video, or Audio.
}
\label{pt_6}
\end{table}

==> tables/table7.tex <==
\begin{table}[ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
\textbf{Dataset Name} & \textbf{Type} & \textbf{I→O} & \textbf{Source}                           & \textbf{Method} & \textbf{\#.Instance} & \textbf{Representative Publications}                                                                             \\ \midrule
LLaVA’s IT~\cite{liu2023llava}            & SFT           & I+T→T        & MS-COCO\cite{lin2014microsoft}                                   & Auto.           & 150K                 & \makecell[c]{MobileVLM~\cite{chu2023mobilevlmv1}, LLaVA-Phi~\cite{zhu2024llava-phi},\\ Mini-Gemini~\cite{li2024mini-gemini}, Vary-toy~\cite{wei2024vary-toy}, \\TinyGPT-V~\cite{yuan2023tinygpt-v}, Imp-v1~\cite{imp2024}, \\ALLaVA~\cite{chen2024allava},SPHINX-X~\cite{gao2024sphinx},\\LLaVA-Gemma~\cite{hinck2024llava-gemma},MM1~\cite{mckinzie2024mm1}} \\ \arrayrulecolor{gray!50} \midrule
ShareGPT4V’s IT\cite{chen2023sharegpt4v}       & SFT           & I+T→T        & \makecell[c]{LCS, COCO~\cite{lin2014microsoft}, SAM~\cite{kirillov2023segment}, \\TextCaps\cite{sidorov2020textcaps}, WikiArt~\cite{saleh2015large}}         & Auto.+Manu.     & –                    & \makecell[c]{Tiny-LLaVA~\cite{zhou2024tinyllava}, Mini-Gemini~\cite{li2024mini-gemini}, \\ MM1~\cite{mckinzie2024mm1}, DeepSeek-VL~\cite{lu2024deepseekvl},\\SPHINX-X~\cite{gao2024sphinx}}                                               \\ \midrule
LLaVA-1.5's IT~\cite{liu2023llava1.5}        & SFT           & I+T→T        & \makecell[c]{LLaVA\cite{liu2023llava},Visual Genome\cite{krishna2017visual},\\ VQAv2\cite{goyal2017vqav2}, ShareGPT\cite{ShareGPT2023}, \\A-OKVQA\cite{schwenk2022okvqa},TextCaps\cite{sidorov2020textcaps}, \\GQA\cite{hudson2019gqa}, OKVQA\cite{marino2019ok},\\OCRVQA, RefCOCO\cite{kazemzadeh2014referitgame, mao2016generation}}   & Auto.+Manu.     & 665K                 & \makecell[c]{Tiny-LLava~\cite{zhou2024tinyllava}, VL-Mamba~\cite{qiao2024vlmamba}, \\Cobra~\cite{zhao2024cobra}, LLaVA-Gemma~\cite{hinck2024llava-gemma}, \\Mipha~\cite{zhu2024mipha}, MoE-LLaVA~\cite{lin2024moe-llava}}                                        \\ \midrule
LRV-Instruct~\cite{liu2023mitigating}          & SFT           & I+T→T        & Visual Genome\cite{krishna2017visual}                             & Auto.           & 300K                 & MoE-LLaVA~\cite{lin2024moe-llava}, Cobra\cite{zhao2024cobra}                                                                                  \\ \midrule
LVIS-INSTRUCT-4V\cite{wang2023see}      & SFT           & I+T→T        & LVIS~\cite{gupta2019lvis}       & Auto.           & 220K                 & \makecell[c]{MoE-LLaVA~\cite{lin2024moe-llava}, SPHINX-X~\cite{gao2024sphinx},\\DeepSeek-VL~\cite{lu2024deepseekvl}, Cobra\cite{zhao2024cobra}}                                                           \\ \midrule
LAION GPT4V\cite{laion2023gpt4v}           & SFT           & I+T→T        & LAION~\cite{schuhmann2021laion}                                     & Auto.           & 12.4k                & \makecell[c]{Mini-Gemini~\cite{li2024mini-gemini}, SPHINX-X~\cite{gao2024sphinx},\\ DeepSeek-VL~\cite{lu2024deepseekvl}}                                                                 \\ \midrule
MiniGPT-4’s IT \cite{zhu2023minigpt4}       & SFT           & I+T→T        & CC3M~\cite{sharma2018conceptual}, CC12M~\cite{changpinyo2021conceptual}                               & Auto.           & 5K                   & TinyGPT-V~\cite{yuan2023tinygpt-v},                                                                                         \\ \midrule
SVIT  \cite{zhao2023svit}                & SFT           & I+T→T        & \makecell[c]{MS-COCO\cite{lin2014microsoft}, \\Visual Genome\cite{krishna2017visual}}                   & Auto.           & 3.2M                 & MoE-LLaVA~\cite{lin2024moe-llava}                                                                                         \\ \midrule
Bunny-695K~\cite{he2024bunny}            & SFT           & I+T→T        & \makecell[c]{SVIT-mix-665K\cite{zhao2023svit}, \\WizardLM-evol-instruct-70K\cite{xu2023wizardlm}} & Auto.     & 695K                 & Bunny~\cite{he2024bunny}                                                                                             \\ \midrule \arrayrulecolor{black}
GQA\cite{hudson2019gqa}                   & SFT             & I+T→T            & Visual Genome\cite{krishna2017visual}                                         & Auto.               &  22M                    & \makecell[c]{MM1~\cite{mckinzie2024mm1}, SPHINX-X~\cite{gao2024sphinx}, \\LLaVA-Gemma~\cite{hinck2024llava-gemma}}                                                        \\ \bottomrule                   
\end{tabular}%
}
\caption{The statistics for common MLLM IT datasets. I→O:Input to Output Modalities,T:Text.}
\label{it_6}
\end{table}
